Fast Shortest Path Polyline Smoothing With $G^1$ Continuity and Bounded Curvature

In this work, we propose a novel and efficient method for smoothing polylines in motion planning tasks. The algorithm applies to motion planning of vehicles with bounded curvature. In the paper, we show that the generated path: 1) has minimal length, 2) is $G^1$ continuous, and 3) is collision-free by construction, if the hypotheses are respected. We compare our solution with the state-of.the-art and show its convenience both in terms of computation time and of length of the compute path.

==> images/data/test1/lengths.tex <==
\def\barwidth{5pt}


% \pgfplotsset{compat=1.18}
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=10pt,
    enlargelimits=0.15,
    ylabel={Ratio},
    xlabel={\# of points}, 
    symbolic x coords={100,10000,100000,1000000},
    xtick=data,
    nodes near coords, 
    nodes near coords align={vertical},
    ylabel near ticks,
    ylabel style={inner sep=0pt},
    ymin=0.9,
    ymax=1.2,
    style={font=\footnotesize},
    legend style={font=\footnotesize}, % Adjust the font size here
]
    \addplot [bar width=\barwidth, bar shift=-2.5pt, fill=orange] table [y=dubinsSeq, col sep=comma]{images/data/test1/lengths.csv};
    \addlegendentry{Sequential}
    \addplot [bar width=\barwidth, bar shift=-7.5pt, fill=blue] table [y=mpdpSaccon, col sep=comma]{images/data/test1/lengths.csv};
    \addlegendentry{MPDP}
    \addplot [bar width=\barwidth, bar shift=+2.5pt, fill=green] table [y=dubinsOmpl, col sep=comma]{images/data/test1/lengths.csv};
    \addlegendentry{OMPL}
    \addplot [bar width=\barwidth, bar shift=+7.5pt, fill=red] table [blue, y=dubinsCuda, col sep=comma]{images/data/test1/lengths.csv};
    \addlegendentry{Parallel}
\end{axis}
\end{tikzpicture}

% \begin{tikzpicture}
% \begin{axis}[
%     ybar,
%     enlargelimits=0.15,
%     legend style={at={(0.5,-0.15)},
%     anchor=north,legend columns=-1},
%     ylabel={Speedup},
%     xlabel={\# of Model Elements (millions)},
%     symbolic x coords={100,10000,100000,1000000},
%     xtick=data,
%     nodes near coords,
%     nodes near coords align={vertical},
%     ]
% \addplot coordinates {(100,92.021) (10000,235.809) (100000,276.824) (1000000,340.847)};
% \addplot table [y=mpdpSaccon, col sep=comma]{images/data/test1/lengths.csv};

% % \addplot coordinates {(100,100.021) (1.5m,230.809) (2m,76.824) (4m,340.847)};
% \end{axis}
% \end{tikzpicture}

==> images/data/test2/fixed_timeout/cactus.tex <==





\begin{tikzpicture}
\begin{axis}[
        xlabel={\# of succesful tests}, 
        ylabel={Sum of lengths},
        ylabel style={inner sep=0pt},
        legend pos=north west,
        legend style={legend columns=-1, font=\footnotesize},
        xtick={0, 20, 40, 60, 80, 100},
        xticklabels={0, 20,  40, 60, 80, 100},
        width=\linewidth,
        height=.6\linewidth,
        font=\small
    ]
    \addplot [Periwinkle, line width=1pt] table [y=Y, x=X, mark=none] {OMPL.tex};
    \addlegendentry{\baseline}
    \addplot [BurntOrange, line width=1pt] table [y=Y, x=X, mark=none] {OMPLPD.tex};
    \addlegendentry{\expOneName}
    \addplot [OliveGreen, line width=1pt] table [y=Y, x=X, mark=none] {RRT.tex};
    \addlegendentry{\expTwoName}
\end{axis}
\end{tikzpicture}

==> images/miterOffset.tex <==
\def\widthConstr{0.2}
\def\widthStruct{1}
\def\widthAxis{0.2}
\def\widthPath{0.75}
\def\widthObsSpace{0.5}

\def\colorObs{red}
\def\colorPolyline{black}
\def\colorStruct{blue}
\def\colorPath{green}

\def\colorOffCircle{BurntOrange}
\def\widthOffCircle{1}

\begin{minipage}[t]{0.48\linewidth}
    \centering
%     \includegraphics[width=\linewidth]{Desmos.PNG}
    \input{images/miterOffset1HgeqR}
    % \input{images/miterOffset1RgeqH}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
    \centering
    \input{images/miterOffset2RgeqH}
    % \vspace{1cm}
    % \input{images/miterOffset2HgeqR}
\end{minipage}
